Do We Really Need to Use Constraint Violation in Constrained Evolutionary Multi-Objective Optimization?

Constraint violation has been a building block to design evolutionary multi-objective optimization algorithms for solving constrained multi-objective optimization problems. However, it is not uncommon that the constraint violation is hardly approachable in real-world black-box optimization scenarios. It is unclear that whether the existing constrained evolutionary multi-objective optimization algorithms, whose environmental selection mechanism are built upon the constraint violation, can still work or not when the formulations of the constraint functions are unknown. Bearing this consideration in mind, this paper picks up four widely used constrained evolutionary multi-objective optimization algorithms as the baseline and develop the corresponding variants that replace the constraint violation by a crisp value. From our experiments on both synthetic and real-world benchmark test problems, we find that the performance of the selected algorithms have not been significantly influenced when the constraint violation is not used to guide the environmental selection.

==> background.tex <==
%!TeX root=main.tex

\section{Preliminaries}
\label{sec:preliminaries}

In this section, we start with some basic definitions closely related to this paper. Then, we give a pragmatic overview of existing works.

\subsection{Basic Definitions}
\label{sec:concepts}

The CMOP considered in this paper is defined as follows:
\begin{equation}
\begin{array}{l l}
\min \quad\quad\quad\, \mathbf{F}(\mathbf{x})=(f_{1}(\mathbf{x}),\cdots,f_{m}(\mathbf{x}))^{T}\\
    \mathrm{subject\ to} \;\;\, \mathbf{g}(\mathbf{x})\leq 0\\
\mathrm{\ } \quad\quad\quad\quad\;\;\, \mathbf{h}(\mathbf{x})=0\\
\mathrm{\ } \quad\quad\quad\quad\;\;\, \mathbf{x}=(x_1,\cdots,x_n)^T\in\Omega
\end{array}
\label{MOP}
\end{equation}
where $\Omega=[x_i^L,x_i^U]^n_{i=1}\subseteq\mathbb{R}^n$ defines the search (or decision variable) space and $\mathbf{x}$ is an $n$-dimensional vector therein. $\mathbf{F}:\Omega\rightarrow\mathbb{R}^m$ constitutes $m$ conflicting objective functions, and $\mathbb{R}^m$ is the objective space. $\mathbf{g}(\mathbf{x})=(g_1(\mathbf{x}),\cdots,g_p(\mathbf{x}))^T$ and $\mathbf{h}(\mathbf{x})=(h_1(\mathbf{x}),\cdots,h_q(\mathbf{x}))^T$ are vectors of inequality and equality constraints respectively.

\begin{definition}
    Given a CMOP, the degree of constraint violation of a solution $\mathbf{x}$ at the $j$-th constraint is calculated as:
    \begin{equation}
        c_i(\mathbf{x})=
        \begin{cases}
            \langle g_j(\mathbf{x})/a_j-1\rangle, & j=1,\cdots,q,\ i=j, \\
            \langle |h_k(\mathbf{x})/b_k-1|-\epsilon\rangle, & k=1,\cdots,p,\ i=k+q,
        \end{cases}
    \end{equation}
    where $\epsilon$ is a small tolerance term (e.g., $\epsilon=10^{-6}$) that relaxes the equality constraints to the inequality constraints. $a_j$ and $b_k$ where $j\in\{1,\cdots,q\}$ and $k\in\{1,\cdots,p\}$ are normalization factors of the corresponding constraints. $\langle\alpha\rangle$ returns 0 if $\alpha\geq 0$ otherwise it returns the negative of $\alpha$.
\end{definition}

\begin{definition}
    Given a CMOP, the constraint violation (CV) value of a solution $\mathbf{x}$ is calculated as:
    \begin{equation}
        CV(\mathbf{x})=\sum_{i=1}^{\ell}c_i(\mathbf{x}),
        \label{eq:cv}
    \end{equation}
    where $\ell=p+q$. $\mathbf{x}$ is feasible in case $CV(\mathbf{x})=0$; otherwise $\mathbf{x}$ is infeasible. 
    \label{def:cv}
\end{definition}

\begin{definition}
    Given two feasible solutions $\mathbf{x}^1$ and $\mathbf{x}^2$, $\mathbf{x}^1$ is said to \textit{Pareto dominate} $\mathbf{x}^2$ (denoted as $\mathbf{x}^1\preceq\mathbf{x}^2$) if and only if $f_i(\mathbf{x}^1)\leq f_i(\mathbf{x}^2)$, $\forall i\in\{1,\cdots,m\}$ and $\exists j\in\{1,\cdots,m\}$ such that $f_i(\mathbf{x}^1)<f_i(\mathbf{x}^2)$.
\end{definition}

\begin{definition}
    A solution $\mathbf{x}^\ast\in\Omega$ is \textit{Pareto-optimal} with respect to (\ref{MOP}) if $\exists\mathbf{x}\in\Omega$ such that $\mathbf{x}\preceq\mathbf{x}^{\ast}$.
\end{definition}

\begin{definition}
    The set of all Pareto-optimal solutions is called the \textit{Pareto-optimal set} (PS). Accordingly, $PF=\{\mathbf{F}(\mathbf{x})|\mathbf{x}\in PS\}$ is called the \textit{Pareto-optimal front} (PF).
\end{definition}

%\begin{definition}
%    The \textit{ideal objective vector} $\mathbf{z}^\ast=(z^\ast_1,\cdots,z^\ast_m)^T$ is constructed by the minimum of each objective functions, i.e., $z^\ast_i=\min_{\mathbf{x}\in\Omega}f_i(\mathbf{x})$, $i\in\{1,\cdots,m\}$.
%\end{definition}
%
%\begin{definition}
%    The \textit{nadir objective vector} $\mathbf{z}^{nad}=(z^{nad}_1,\cdots,z^{nad}_m)^T$ is constructed by the worst objective functions of the PF, i.e., $z^{nad}_i=\max_{\mathbf{x}\in PS}f_i(\mathbf{x})$, $i\in\{1,\cdots,m\}$.
%\end{definition}

\subsection{Related Works}
\label{sec:literature}

In the 90s, some early endeavors to the development of EAs for solving CMOPs (e.g.,~\cite{FonsecaF98} and~\cite{CoelloC99}) are simply driven by a prioritization of the search for feasible solutions over \lq optimal\rq\ one. However, such methods are notorious for the loss of selection pressure in case the population is filled with infeasible solutions.

After the development of the constrained dominance relation~\cite{DebAPM02}, most, if not all, prevalent constraint handling techniques in the EMO community directly or indirectly depend on the CV defined in~\pref{def:cv}. Specifically, a solution $\mathbf{x}^1$ is said to constraint-dominate $\mathbf{x}^2$, if: 1) $\mathbf{x}^1$ is feasible while $\mathbf{x}^2$ is not; 2) both of them are infeasible and $CV(\mathbf{x}^1)<CV(\mathbf{x}^2)$; or 3) both of them are feasible and $\mathbf{x}^1\prec\mathbf{x}^2$. By replacing the Pareto dominance relation with this constrained dominance relation, the state-of-the-art NSGA-II and NSGA-III~\cite{JainD14} can be readily used to tackle CMOPs. Borrowing this idea, several MOEA/D variants (e.g.,~\cite{JanZ10,JainD14,ChengJOS16,LiuWH20}) use the CV as an alternative criterion in the subproblem update procedure. Moreover, the constrained dominance relation is augmented with terms such as the number of violated constraints~\cite{OyamaSF07}, $\epsilon$-constraint~\cite{TakahamaS12,MartinezC14,AsafuddoulaRS15} and angle between each other~\cite{FanLCHLL16} to provide an additional selection pressure to infeasible solutions whose CV values have a marginal difference.

In addition to the above feasibility-driven constraint handling techniques, the second category aims at balancing the trade-off between convergence and feasibility during the search process. For example, Jim\'enez et al.~\cite{JimenezGSD02} proposed a min-max formulation that drives feasible and infeasible solutions evolve towards optimality and feasibility, respectively. In~\cite{RayTS01}, a Ray-Tai-Seow algorithm was proposed to simultaneously take the objective values, the CV along with the combination of them into consideration to compare and rank non-dominated solutions. Based on the similar rigour, some modified ranking mechanisms (e.g.,~\cite{Young05,AngantyrAA03,WoldesenbetYT09}) were developed by leveraging the information from both the objective and constraint spaces. Instead of prioritizing feasible solutions, some researchers (e.g.,~\cite{LiDZK15,PengLG17,SorkhabiAK17}) proposed to exploit information from infeasible solutions in case they can provide additional diversity to the current evolutionary population.

As a step further, the third category seeks to strike a balance among convergence, diversity and feasibility simultaneously. As a pioneer along this line, Li et al. proposed a two-archive EA (C-TAEA) that maintains two co-evolving and complementary populations to solve CMOPs~\cite{LiCFY19}. Specifically, one archive, denoted as the convergence-oriented archive (CA), pushes the population towards the PF; while the other one, denoted as the diversity-oriented archive, provides additional diversity. To complement the behavior of the CA, the DA explores the areas under-exploited by the CA including the infeasible region(s). In addition, to take advantage of the complementary effects of both CA and DA, a restricted mating selection mechanism was proposed to adaptively choose appropriate mating parents according to the evolution status of the CA and DA respectively. After C-TAEA, there have been a spike of efforts on the development of multi-population strategies (e.g.,~\cite{ShanL21,TianZXZJ21,LiuWT21,WangLZZG21,MingGWG22,MingGWL22}) to leverage some complementary effects of both feasible and infeasible solutions simultaneously for solving CMOPs.

Instead of the environmental selection, the last category tries to repair the infeasible solutions in order to drives them towards the feasible region(s). For example, a so-called Pareto descent repair operator~\cite{HaradaSOK06} was proposed to explore possible feasible solutions along the gradient information around infeasible solutions in the constraint space. In~\cite{JiaoLSL14}, a feasible-guided strategy was developed to guide infeasible solutions towards the feasible region along the \lq feasible direction\rq, i.e., a vector starting from an infeasible solution and ending up with its nearest feasible solution. In~\cite{SinghRS10}, a simulated annealing was applied to accelerate the progress of movements from infeasible solutions toward feasible ones.

\begin{remark}
    As discussed at the outset of this subsection, all these prevalent constraint handling techniques require the access of the CV. This applies to the last category, since it needs to access the gradient information of the CV. The implicit assumption behind the prevalent constraint handling techniques is the access of the closed form of the constraint function(s). However, this is not practical since real-world optimization scenarios are usually as a black box. In other words, we can only know that whether a solution is feasible or not.
\end{remark}
Bearing this consideration in mind, we come up with the overarching research question of this paper: \textit{do the prevalent constraint handling techniques in the EMO literature still work when we do not have an access to the CV?}


